NOMAD-EEG: Native Omni-Montage Adaptive Diffusion

Purpose. Electroencephalography (EEG) montages, channel counts and recording lengths vary widely, but most EEG foundation models are bound to the channel set and input length they were trained on. We aimed to build a generative EEG foundation model independent of the number, identity and order of electrodes and of the input length. Methods. NOMAD-EEG is a 12.0 M-parameter diffusion model that alternates state-space layers along time, without patches, with attention across electrodes identified only by their 3D scalp position. It was pre-trained on 147 h of unlabelled EEG from a single corpus and evaluated with frozen linear probes on ten datasets with 1 to 64 electrodes against seven foundation models run under one protocol, and on two unseen populations. Results. Despite its small size (12.0 M parameters against 69 M for REVE) and single pre- training corpus, NOMAD-EEG outperformed all seven foundation models on EEGMMIDB mo- tor imagery (balanced accuracy 0.442), Siena seizure detection (macro F1 0.622) and Bonn seizure detection (AUROC 0.999), had the highest accuracy of the seven compared models on TUEP epilepsy diagnosis (0.640) and, after fine-tuning, the highest \k{appa} (0.635) and weighted F1 (0.814) on TUEV event classification. It was the best of five models on P300 detection in autism with an unseen eight-electrode montage (AUROC 0.718). With only 5 of 19 electrodes, its mean AUROC fell only from 0.942 to 0.891. Conclusion. Identifying electrodes by position and modelling time without patches let one small model, pre-trained on one corpus, outperform much larger EEG foundation models on seizure detection, epileptiform event classification, epilepsy diagnosis and motor imagery.

==> sections/old/ablations.tex <==
\section{Ablations}
\label{sec:ablations}

\subsection{Does pre-training help?}

To separate what pre-training contributes from what the architecture and the task head contribute, we
evaluate the same network with random weights through the identical feature extraction and protocol
(\cref{tab:pretrain}). Pre-training improves balanced accuracy on TUEV by 0.107 as a frozen probe and
by 0.132 after fine-tuning, improves TUAB AUROC by 0.040, and improves Siena macro F1 by 0.071, all
with non-overlapping confidence intervals. Two results show where it does not help. On Siena, the
gain is in precision at the decision threshold (macro F1; PR-AUC is also higher, but its CIs
overlap) and not in ranking: AUROC is unchanged. On Mumtaz, fine-tuning
from random weights matches fine-tuning from the pre-trained model, which suggests that this small,
two-class task is solvable by the architecture alone. Bonn is saturated for both. The random-weights
control is strong on some tasks, which is why we report it rather than assume that pre-training
explains every result.

\input{tables/pretrain}

\subsection{Diffusion or flow matching?}

Recent work has proposed flow matching as a more sample-efficient generative pre-training objective
for EEG~\citep{hwang2026bfm}. Because the objective is a single switch in our implementation, we
trained a second model, \model{}-F, that differs from \model{}-D only in the objective (rectified
flow, \cref{sec:objective}) and compared the two on every downstream dataset with a paired bootstrap
on the shared test samples (\cref{tab:objective}). Diffusion is better on four datasets (TUEV, TUAB,
Siena macro F1 and Sleep-EDF), flow is better on one (TUSZ balanced accuracy, by 0.011), and the
remaining comparisons show no difference. The largest gaps favour diffusion: 0.055 balanced accuracy
on TUEV and 0.041 on Sleep-EDF. In our architecture and at our data scale, the denoising objective
therefore gives better frozen representations, and we use it for \model{}.

\input{tables/objective}

\subsection{Electrode order and missing electrodes}
\label{sec:missing}

\Cref{sec:properties} shows that \model{} is equivariant to the order of its electrodes by
construction. We confirmed this on the Mumtaz test set (19 electrodes, 1{,}179 windows): with the
electrodes listed in five random orders, each keeping its own position, every gate activation
equals the original with its rows permuted (largest relative difference $5.6\times10^{-6}$,
floating-point rounding), and no test prediction changes. As a control, shuffling the positions
while leaving the signals in place changes 17.5\% of the predictions and lowers AUROC from 0.942
to 0.909, so the invariance does not come from ignoring spatial information.

In practice electrodes are also lost, through poor contact or a smaller cap. Because \model{} reads any set of positions, a recording with
electrodes removed needs no imputation and no change to the model. We test this on the Mumtaz test
set: the linear probe is trained once on the full 19-electrode montage and applied, unchanged, to
the same test recordings with only 14, 10 or 5 electrodes given, five random subsets for each
size (\cref{fig:missing}). The model's ranking of the test windows is largely preserved: the mean
AUROC falls from 0.942 with all electrodes to 0.919 with 14, 0.919 with 10 and 0.891 with 5, and
no subset falls below 0.877. Balanced accuracy at the probe's fixed threshold degrades more: it
stays at 0.826 on average with 14 electrodes but falls to 0.774 with 10 and 0.696 with 5, and to
chance (0.501) for one five-electrode subset (Fp1, F7, T5, Fz, Pz) whose AUROC is still 0.877.
Removing electrodes therefore leaves the scores well ordered but shifts them relative to the
threshold learned on the full montage, because the probe reads the average over electrodes. A
threshold recalibrated on the reduced montage, or a probe trained with electrodes dropped at
random, would address this. Base was pre-trained on a single 21-electrode montage and never saw
a reduced one; \model{}-Large is pre-trained on random electrode subsets of 2 to 32 electrodes (\cref{sec:scaling}).

\begin{figure}[!tp]
  \centering
  \includegraphics[width=\textwidth]{figures/fig6_channel_subset.pdf}
  \caption{\textbf{Missing-electrode test on Mumtaz} (1{,}179 test windows). The linear probe is
  trained once on the full montage and applied unchanged. (a) Each scalp shows one test condition:
  filled dots are the electrodes given to the model, hollow dots those removed; the shading and the
  label give the AUROC, and BAcc is the balanced accuracy at the probe's threshold. Rows: 19, 14,
  10 and 5 electrodes; columns: five random subsets per size. (b) The same results against the
  number of electrodes given: dots are individual subsets, lines the mean, bands the range over
  subsets. AUROC stays high as electrodes are removed, while balanced accuracy drops because the
  scores shift relative to the threshold fitted on the full montage.}
  \label{fig:missing}
\end{figure}

\subsection{What does the model respond to?}
\label{sec:attribution}

To see what drives \model{}'s seizure decisions, we fed it one seizure and one normal 5\,s segment
from the TUSZ test set, whose patients the probe never saw, and computed which parts of the input
raised the seizure score (Integrated Gradients of the probe's logit with respect to the input, with
every channel at its median as the baseline). In the seizure segment, the evidence concentrates on
the sharp, high-amplitude discharges, and its time course peaks where they occur; in the normal
segment there is almost no evidence anywhere (\cref{fig:attribution}).

\begin{figure}[!htbp]
  \centering
  \includegraphics[width=\textwidth]{figures/fig_example_attribution.pdf}
  \caption{\textbf{Where \model{} finds evidence of a seizure.} Two 5\,s segments from the TUSZ test
  set, scored by the frozen \model{} with the TUSZ linear probe of \cref{tab:tusz}. The segments were
  chosen by a rule fixed in advance: a random (seeded) test window labelled seizure that the model
  classifies with probability above 0.9, and a random normal window classified with probability
  below 0.1, i.e.\ typical correct decisions rather than hand-picked ones. Shading behind each trace:
  positive Integrated-Gradients attribution (evidence for seizure) per electrode and 0.25\,s; bottom:
  its sum over electrodes. Both panels share the colour and amplitude scales. The figure illustrates
  single decisions and is not a quantitative test of seizure localisation.}
  \label{fig:attribution}
\end{figure}


==> sections/old/scaling.tex <==
\section{Scaling model size and pre-training data}
\label{sec:scaling}

\model{} was pre-trained on 147\,h from one corpus with one montage. To test whether the
architecture improves when it is made larger and given more, and more varied, EEG, we trained
\model{}-Large, which scales the model and the pre-training data together, and evaluated it with
exactly the protocols used for Base.

\paragraph{Model.}
\model{}-Large uses the same code and the same block as Base (\cref{sec:arch}), widened
from $d=256$ to $d=512$, deepened from 16 to 24 blocks and given 8 instead of 4 attention heads:
67.6\,M parameters against 12.0\,M (5.6$\times$). Features are read from blocks 6, 12, 18 and 24
with the same windowed mean and standard deviation, which gives 20{,}480 dimensions instead of
10{,}240 (\cref{tab:scaling_setup}).

\paragraph{Pre-training data.}
The pool contains 6{,}984\,h of EEG from seven corpora (47$\times$ Base): Sleep-EDF expanded
(2{,}954\,h), TUSZ (1{,}202\,h, training and development splits), TUAB (1{,}024\,h, training split),
CHB-MIT (990\,h), TUEP (627\,h), TUEV (147\,h, as for Base) and SEED-V (41\,h). Recordings keep their
native montages, with every channel that has a standard 10-20 or 10-05 position (bipolar
derivations at the midpoint of their two electrodes), which gives 38 distinct channel groups with up
to 62 electrodes. Signals are resampled to 200\,Hz and cut into 30\,s windows, and each window's
per-channel median is removed. The evaluation patients of TUSZ and TUAB and the Sleep-EDF subjects
used downstream were held out of the pool, as were Siena, Bonn, Mumtaz, EEGMMIDB and BCIAUT. TUEP
and SEED-V were included in full, so for Large these two evaluations are in-domain.

\paragraph{Training.}
Each batch is drawn from one channel group, with a random subset of 2 to 32 of its electrodes and a
crop of 30\,s half of the time and 5 to 25\,s otherwise, capped at 640 electrode-seconds per sample.
Corpora are sampled with probability proportional to $\sqrt{\min(\text{hours},1{,}200)}$, so the
largest corpora do not dominate. The optimiser, schedule, moving average, precision and effective
batch of 32 are those of Base (\cref{sec:impl}), with learning rate $2\times10^{-4}$ and a
2{,}000-step warm-up, for a planned 60{,}000 steps. Large was trained on a single 20\,GB slice of an
A100 GPU (4 samples per step with 8-step gradient accumulation) in 12-hour jobs that resume from the
last checkpoint. We report two checkpoints, at 27{,}000 and 51{,}000 steps; at step 51{,}000 the
learning rate has decayed to 5\% of its peak.

\begin{table}[!htbp]
\centering
\caption{Base and Large configurations. Passes over the pool are an upper bound for Large, whose
samples are at most 30\,s long.}
\label{tab:scaling_setup}
\small
\begin{tabular}{@{}l c c@{}}
\toprule
 & \model{} (Base) & \model{}-Large \\
\midrule
Parameters & 12.0\,M & 67.6\,M \\
Width / blocks / heads & 256 / 16 / 4 & 512 / 24 / 8 \\
Feature dimension & 10{,}240 & 20{,}480 \\
Pre-training data & 147\,h, 1 corpus & 6{,}984\,h, 7 corpora \\
Montages & 1 (21 electrodes) & 38 channel groups, 1--62 electrodes \\
Electrodes per sample & 21 & random subset of 2--32 \\
Steps $\times$ effective batch & 40{,}000 $\times$ 32 & 51{,}000 $\times$ 32 (of 60{,}000) \\
Samples seen & 1.28\,M & 1.63\,M \\
Passes over the pool & $\approx$72 & $\le$2 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Results.}
\Cref{tab:scaling} compares the two models on all ten benchmarks with each dataset's primary metric.
At step 51{,}000, \model{}-Large is not better than Base on any dataset: no Large interval lies above
Base's. Its interval lies entirely below Base's on EEGMMIDB (balanced accuracy 0.361 against 0.442),
Sleep-EDF (0.724 against 0.757) and SEED-V (0.301 against 0.315). It is lower, with intervals that
overlap or just touch, on TUSZ (AUROC 0.856 against 0.866) and Mumtaz (0.913 against 0.942). It is
level on Bonn (1.000 against 0.999), TUAB (0.837 against 0.838), TUEV (balanced accuracy 0.542 against
0.542) and TUEP (patient AUROC 0.694 against 0.679; paired difference 95\% CI $[-0.061, 0.031]$).
The highest Large value relative to Base is TUSZ at step 27{,}000 (AUROC 0.878 against
0.866, overlapping intervals), which fell below Base by step 51{,}000. Between the two checkpoints
Large improved on TUEV (0.450 to 0.542), EEGMMIDB (0.326 to 0.361), TUEP (0.658 to 0.694) and TUAB
(0.828 to 0.837), and changed little elsewhere.

\input{tables/scaling}

\paragraph{Findings.}
\begin{enumerate}
  \item \textbf{Scaling model and data together did not improve the frozen features.} With
  5.6$\times$ the parameters and 47$\times$ the pre-training data, \model{}-Large was not better
  than Base on any benchmark at its latest checkpoint, and was clearly worse on three.
  \item \textbf{The largest losses are on the tasks least like clinical EEG.} Motor imagery
  (EEGMMIDB, $-0.081$ balanced accuracy), sleep staging (Sleep-EDF, $-0.033$), emotion (SEED-V,
  $-0.014$) and depression (Mumtaz, $-0.029$ AUROC) lose most, although Large was pre-trained on many
  montages, on random electrode subsets and, for SEED-V and Sleep-EDF, on the same corpora.
  \item \textbf{Seeing the evaluation corpus in pre-training did not help.} SEED-V and TUEP were in
  Large's pre-training data and not in Base's, yet Large is below Base on SEED-V and level on TUEP.
  \item \textbf{Longer training does not improve every task.} From step 27{,}000 to 51{,}000 TUEV and
  EEGMMIDB improved while TUSZ dropped from above Base's point estimate to below it, so a single
  intermediate checkpoint can over- or understate a model.
  \item \textbf{The compute was not scaled with the data.} Large saw 1.63\,M samples against Base's
  1.28\,M, which is at most two passes over its pool against about 72 passes for Base over TUEV. Large
  may therefore be under-trained relative to its data, and its features are twice as wide for the same
  linear probe. We have not tested which of these explains the result; a study that
  scales compute with model and data, and that varies model size and data size separately, is needed
  before concluding that this architecture does not benefit from scale.
\end{enumerate}


==> sections/old/zeroshot.tex <==
\section{Transfer to unseen populations: P300 detection in autism and Parkinson's disease}
\label{sec:zeroshot}

To test whether \model{} transfers to a population, task and montage that none of the models
saw in pre-training, we evaluate frozen encoders on BCIAUT-P300~\citep{simoes2020bciaut}. No
encoder is trained or fine-tuned on any data from this corpus: the pre-trained weights are used
as they are, and only a linear classifier is fitted on top (a linear probe), always on subjects
other than the ones it is tested on.

\paragraph{Data.}
BCIAUT-P300 contains EEG from 15 young people with autism spectrum disorder (ASD), each recorded
in 7 sessions of a P300-based brain--computer-interface training in which eight objects are
flashed and the participant attends to one of them~\citep{simoes2020bciaut}. EEG was recorded at
250\,Hz from eight electrodes (C3, Cz, C4, CPz, P3, Pz, P4, POz) and epoched from $-200$ to
1{,}200\,ms around each flash. Because every participant has ASD, the task is \emph{not} autism
diagnosis but P300 detection: deciding whether a flashed object was the attended target. We use
the labelled calibration data of every session: 20 blocks of 10 runs of 8 flashes, 1{,}600 epochs
per session and 168{,}000 epochs in total, of which 21{,}000 (12.5\%) are targets. Epochs are
resampled to 200\,Hz (280 samples, 1.4\,s) and normalised per channel with a median and
inter-quartile range pooled over all epochs without using labels, then clipped at $\pm20$.
The Kaggle release also contains labels for the online (test) sessions, which were withheld in
the original challenge; we do not use them.

\paragraph{Models and inputs.}
We compare \model{}-D with DiffEEG~\citep{diffeeg2026}, EEGDM~\citep{puah2025eegdm},
REVE~\citep{ouahidi2025reve} and BIOT~\citep{yang2023biot}, each fed in its native input format
(\cref{sec:related}). This montage is new to all five models, and they can read different
amounts of it. \model{} and REVE place all eight electrodes by their 3D positions; CPz and POz
are not in \model{}'s pre-training montage. DiffEEG's fixed 22-channel layout has slots for six
of the eight (C3, Cz, C4, P3, Pz, P4). EEGDM's vocabulary of bipolar channels allows four
derivations (C3--Cz, C4--Cz, C3--P3, C4--P4), and BIOT's allows two (C3--P3, C4--P4). Two models
also need an adaptation to the 1.4\,s epoch. EEGDM pools its gate activations over one window
spanning the whole epoch instead of 1\,s windows. REVE keeps its own 1\,s patches, so it reads a
single patch covering $-200$ to 800\,ms, which contains the P300 (typically 250--500\,ms after the
flash).

\paragraph{Protocol.}
Features are extracted once with each frozen encoder (for \model{}, the frozen feature extractor of
\cref{sec:readouts}). The 15 subjects are split into five folds of three (subject-grouped
cross-validation). In each fold, a class-balanced, L2-regularised logistic regression is trained
on the other twelve subjects; its strength $C\in\{10^{-4},\dots,10\}$ is chosen by AUROC on three
of those twelve held out as validation, and the classifier is then refitted on all twelve and
applied to the three test subjects. Every epoch is therefore predicted exactly once, by a
classifier that never saw its subject. We report, on the pooled out-of-fold predictions,
AUROC, balanced accuracy and PR-AUC (chance level equals the target rate, 0.125), with 95\%
confidence intervals from 1{,}000 bootstrap resamples of subjects. We also report the decision a
P300 speller actually makes: in each block, the object whose flashes receive the highest mean
target probability over the first $k$ runs is selected, and we score how often it is the
attended object (chance 12.5\%) for $k=1$, 3 and 10.

\paragraph{Results.}
\model{} is the best of the five models on every metric (\cref{tab:bciaut}). It reaches an AUROC
of 0.718 and selects the attended object in 75.5\% of blocks after ten runs, against 61.2\% for
EEGDM and 57.5\% for REVE. The advantage holds within subjects: its per-subject AUROC exceeds REVE's in all 15 subjects
and EEGDM's in 13. BIOT and DiffEEG are close to chance. We
attribute this mainly to how little of the montage they can read: two bipolar pairs for BIOT,
and six of eight electrodes for DiffEEG. Bipolar derivations also cancel part of a P300 that is
broad and similar across these closely spaced electrodes.

\begin{table}[t]
\centering
\caption{P300 detection on BCIAUT-P300 (15 participants with ASD, 168{,}000 epochs,
12.5\% targets). Encoders are frozen and never trained on this corpus; a linear probe is
evaluated on subjects it never saw (five folds of three subjects). Brackets: 95\% CI from a
bootstrap over subjects. ``Object acc.'' is the rate at which the attended object among eight is
selected from the first 1, 3 or 10 runs of a block (chance 12.5\%).}
\label{tab:bciaut}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l c l c c c c@{}}
\toprule
Model & Channels read & AUROC & Bal.\ acc. & PR-AUC & Object acc.\ (1/3/10 runs) & Per-subject AUROC range \\
\midrule
\textbf{\model{}-D} & 8 & \textbf{0.718} [0.695, 0.739] & \textbf{0.660} & \textbf{0.289} & \textbf{32.6 / 51.5 / 75.5\%} & 0.652--0.805 \\
EEGDM & 4 bipolar & 0.667 [0.631, 0.699] & 0.624 & 0.227 & 27.8 / 42.4 / 61.2\% & 0.540--0.805 \\
REVE & 8 & 0.651 [0.626, 0.675] & 0.612 & 0.209 & 24.6 / 37.9 / 57.5\% & 0.563--0.752 \\
BIOT & 2 bipolar & 0.530 [0.521, 0.539] & 0.520 & 0.136 & 14.5 / 17.2 / 21.8\% & 0.503--0.571 \\
DiffEEG & 6 & 0.522 [0.508, 0.534] & 0.517 & 0.133 & 13.9 / 15.1 / 19.4\% & 0.457--0.556 \\
\bottomrule
\end{tabular}}
\end{table}


\todo{The probe selected the smallest $C$ in the grid ($10^{-4}$) for \model{} in all five folds;
decide whether to extend the grid for all models before the final version.}

\subsection{Parkinson's disease}
\label{sec:parkinson}

\paragraph{Data and protocol.}
We apply the same unseen-participant protocol to a diagnostic task: Parkinson's disease (PD) against
healthy controls in OpenNeuro ds004584, 149 participants (100 PD, 49 controls) recorded at rest
with eyes open for about two minutes with a 64-channel cap at 500\,Hz. We keep the 60 electrodes
that have a standard 10-05 position and are present in every recording, convert to microvolts,
resample to 200\,Hz, remove each window's per-channel median and cut 5\,s windows (4{,}719 in
total). The 149 participants are split into five folds stratified by group, identical for every
model; in each fold the logistic regression's $C\in\{10^{-9},\dots,10\}$ is chosen by AUROC on 20\%
of the training participants, and the classifier is refitted on all training participants. The
diagnosis is made per participant, as the mean probability of their windows; confidence intervals
resample participants.

\paragraph{Results.}
All five models detect Parkinson's disease above chance from frozen features, but here \model{} is
not the best (\cref{tab:parkinson}). EEGDM reaches a participant-level AUROC of 0.795
[0.714, 0.868], significantly above \model{}'s 0.684 [0.590, 0.777] (paired difference
$-0.111$, 95\% CI $[-0.203, -0.012]$); \model{} is level with BIOT, DiffEEG and REVE, whose
intervals overlap its own. \model{}'s selected $C$ ranged from $10^{-4}$ to 10 across folds, a sign
that its probe is unstable with about 24 validation participants per fold. One possible reason for
the gap, which we have not tested, is that the resting-state changes reported in PD are spectral
properties of the whole recording rather than transient events like those in \model{}'s
pre-training data.

\input{tables/parkinson}


==> tables/ranks.tex <==
\begin{table}[!htbp]
\centering
\caption{Rank of each model (1 = best of eight) on the primary metric of each dataset: AUROC for binary tasks, balanced accuracy for multi-class tasks. Frozen linear probes throughout.}
\label{tab:ranks}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l c c c c c c c c c@{}}
\toprule
Model & TUAB & TUSZ & TUEV & Siena & Bonn & Mumtaz & EEGMMIDB & Sleep-EDF & Mean rank \\
\midrule
REVE & \textbf{1} & \textbf{1} & 2 & 2 & 2 & \textbf{1} & 3 & 2 & 1.75 \\
EEGDM & 2 & 2 & \textbf{1} & \textbf{1} & 5 & 2 & 4 & \textbf{1} & 2.25 \\
\model{} & 4 & 3 & 3 & 3 & \textbf{1} & 3 & \textbf{1} & 3 & 2.62 \\
LaBraM & 6 & 5 & 4 & 6 & 4 & 5 & 7 & 5 & 5.25 \\
CBraMod & 5 & 4 & 7 & 5 & 3 & 8 & 5 & 6 & 5.38 \\
BIOT & 3 & 8 & 6 & 8 & 7 & 4 & 8 & 4 & 6.00 \\
EEGMamba & 8 & 6 & 5 & 4 & 8 & 7 & 6 & 7 & 6.38 \\
DiffEEG & 7 & 7 & 8 & 7 & 6 & 6 & 2 & 8 & 6.38 \\
\bottomrule
\end{tabular}
\end{table}

